Position: How Regulation Will Change Software Security Research

Software security has been an important research topic over the years. The community has proposed processes and tools for secure software development and security analysis. However, a significant number of vulnerabilities remains in real-world software-driven systems and products. To alleviate this problem, legislation is being established to oblige manufacturers, for example, to comply with essential security requirements and to establish appropriate development practices. We argue that software engineering research needs to provide better tools and support that helps industry comply with the new standards while retaining effcient processes. We argue for a stronger cooperation between legal scholars and computer scientists, and for bridging the gap between higher-level regulation and code-level engineering.

==> text/conformity.tex <==
%The CRA defines different categories of products, depending on their criticality. A vulnerability in an operating system may have a much more severe effect than a vulnerability in a mobile gaming app. For each category, the CRA regulates which procedures for conformity assessment may be used.

%The first category is called \emph{important products} and is sub-divided into two \emph{classes}. The first class contains, among others, identity management systems, browsers, password managers, anti-malware tools and VPN products. The second class contains hypervisors for virtualiztion, firewalls and tamper-resistant components. The second category is called \emph{critical products} and contains hardware security modules and smartcards. Note that all categories can be extended by the European Commission.

%The conformity assessment procedures are structured into \emph{modules}. We argue that these modules require tool support and process beyond what is currently available as we show in the remainder of this section.

%\paragraph{Module A} is a self-assessment by the manufacturer who declares that their processes ensure compliance with the requirements of the CRA. The entire responsibility for product security and CRA compliance lies with the manufacturer in this module. Currently, the outputs of individual language- or platform-specific code analyses and security frameworks need to be combined and aligned with the risk model by hand. The manfacturer must provide their own justification as to why the chosen approach is sufficient to mitigate the risks and place on the market a product without security vulnerabilities that are (or should have been) known to the manufacturer. The software security community should establish best practices, along with suitable tooling, moving towards standardization.



